Knowledge Sheaves: A Sheaf-Theoretic Framework for Knowledge Graph Embedding

Knowledge graph embedding involves learning representations of entities -- the vertices of the graph -- and relations -- the edges of the graph -- such that the resulting representations encode the known factual information represented by the knowledge graph and can be used in the inference of new relations. We show that knowledge graph embedding is naturally expressed in the topological and categorical language of \textit{cellular sheaves}: a knowledge graph embedding can be described as an approximate global section of an appropriate \textit{knowledge sheaf} over the graph, with consistency constraints induced by the knowledge graph's schema. This approach provides a generalized framework for reasoning about knowledge graph embedding models and allows for the expression of a wide range of prior constraints on embeddings. Further, the resulting embeddings can be easily adapted for reasoning over composite relations without special training. We implement these ideas to highlight the benefits of the extensions inspired by this new perspective.

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/commands.tex <==
\usepackage{amsmath,amsfonts,amssymb,bm}
\usepackage{stmaryrd}
\DeclareMathOperator{\Tr}{Tr}

\newcommand{\env}{\text{env}}
\renewcommand\vec{\bm}
\newcommand{\mat}[1]{{\bm{#1}}}
\newcommand{\lap}{{\mat{\mathcal{L}}}}

% blackboard bold for naturals, integers, etc.
\newcommand{\N}{\mathbb{N}}
% \newcommand{\Z}{\mathbb{Z}}
% \newcommand{\Q}{\mathbb{Q}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\C}{\mathbb{C}}

%comments shown
\newcommand{\paul}[1]{\textcolor{red}{(Paul says: {#1})}}
\newcommand{\tom}[1]{\textcolor{blue}{(Tom says: {#1})}}

\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}

%Geometry/Topology
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\maxidx}{maxidx}
\DeclareMathOperator{\Co}{Co}
\DeclareMathOperator{\face}{\trianglelefteqslant}
\DeclareMathOperator{\faceone}{\trianglelefteqslant_1}
\DeclareMathOperator{\st}{st}
\newcommand{\realize}[1]{\left\lvert#1\right\rvert}
\DeclareMathOperator*{\argmin}{arg\,min}

% Variables for sheaves
\newcommand{\shfa}{\Fc}
\newcommand{\shfb}{\Gc}
\newcommand{\shfc}{\mathcal{E}}
\newcommand{\constshf}[1]{\underline{#1}}
\newcommand{\constcoshf}[1]{\overline{#1}}
\newcommand{\bundlea}{\shfa}
\newcommand{\bundleb}{\shfb}
\newcommand{\coshfa}{{\hat{\Fc}}}
\newcommand{\coshfb}{{\hat{\shfb}}}
\newcommand{\appshf}[1]{{#1}'}

% Laplacians
\newcommand{\upL}[1]{\Delta^{#1}_{+}}
\newcommand{\downL}[1]{\Delta^{#1}_{-}}
\newcommand{\Lap}[1]{\Delta^{#1}}
\newcommand{\nL}{\mathcal{L}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}


==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/both/vs_baselines_mrr.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
    \hline
        dataset & model & 1p & 2p & 3p & 2i & 3i & pi & ip & parameters (M) \\ \hline
        FB15k-237 & BetaE & 0.390 & 0.109 & 0.100 & 0.288 & 0.425 & 0.224 & 0.126 & 14.3 \\ 
        ~ & Q2B & 0.406 & 0.094 & 0.068 & 0.295 & 0.423 & 0.212 & 0.126 & 6.8 \\ 
        ~ & GQE & 0.350 & 0.072 & 0.053 & 0.233 & 0.346 & 0.165 & 0.107 & 13.3 \\ \cline{2-10}
        ~ & ExtensionSE & 0.197 & 0.024 & 0.013 & 0.085 & 0.110 & 0.055 & 0.040 & 1.4 \\ 
        ~ & ExtensionTransE & 0.207 & 0.027 & 0.021 & 0.071 & 0.103 & 0.045 & 0.047 & 0.5 \\ \hline
        NELL & BetaE & 0.530 & 0.130 & 0.114 & 0.376 & 0.475 & 0.241 & 0.143 & 53.4 \\
        ~ & Q2B & 0.422 & 0.140 & 0.112 & 0.333 & 0.445 & 0.224 & 0.168 & 26.3 \\ 
        ~ & GQE & 0.328 & 0.119 & 0.096 & 0.275 & 0.352 & 0.184 & 0.144 & 52.3 \\ \cline{2-10}
        ~ & ExtensionSE & 0.159 & 0.037 & 0.024 & 0.109 & 0.118 & 0.125 & 0.072 & 2.8 \\ 
        ~ & ExtensionTransE & 0.187 & 0.035 & 0.028 & 0.083 & 0.079 & 0.088 & 0.069 & 2.0 \\ \hline
    \end{tabular}
\caption{Performance of logical query baselines versus the harmonic extension solution for simple StructuredEmbedding and TransE models using the evaluation setup of \citet{ren2020beta}. The first seven columns measure MRR performance for each complex query structure while the final column measures the number of trainable parameters (in millions). The Extension models set $\dim \mathcal{F}(s) = \dim \mathcal{F}(r) = 32$ and contain one section. Performance metrics for BetaE, Q2B, and GQE models taken from \citet{ren2020beta}.}
\label{tab:vs_baselines_mrr}
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/easy/naive_vs_extension_hits_at_10.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        dataset & model & 2p & 3p & 2i & 3i & pi & ip \\ \hline
        NELL-995 & ExtensionTransE & 0.355 & 0.201 & 0.467 & 0.368 & 0.499 & 0.427 \\
        ~ & NaiveTransE & 0.280 & 0.148 & 0.488 & 0.403 & 0.451 & 0.216 \\ \hline
        FB15k-237 & ExtensionTransE & 0.163 & 0.107 & 0.343 & 0.341 & 0.253 & 0.207 \\
        ~ & NaiveTransE & 0.162 & 0.095 & 0.362 & 0.363 & 0.229 & 0.097 \\ \hline
\end{tabular}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/easy/naive_vs_extension_mrr.tex <==
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
    dataset & model & 2p & 3p & 2i & 3i & pi & ip \\ \hline
    NELL-995 & ExtensionTransE & \textbf{0.237} & \textbf{0.120} & 0.280 & 0.198 & \textbf{0.340} & \textbf{0.296} \\
    ~ & NaiveTransE & 0.164 & 0.082 & \textbf{0.281} & \textbf{0.205} & 0.271 & 0.104 \\ \hline
    FB15k-237 & ExtensionTransE & \textbf{0.084} & 0.050 & 0.157 & 0.147 & \textbf{0.119} & \textbf{0.109} \\ 
    ~ & NaiveTransE & 0.079 & \textbf{0.052} & \textbf{0.163} & \textbf{0.167} & 0.107 & 0.049 \\ \hline
\end{tabular}}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/fb15k-237_1.tex <==
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Multisection}  & 16                   & 1                   & 0          & 4.03  & 0.03 & 0.04 & 0.2  & 0.15 & 0.01 & 0.01 \\ \cline{2-11} 
                                & 32                   & 1                   & 0          & 4.65  & 0.01 & 0.02 & 0.28 & 0.18 & 0.01 & 0.01 \\ \cline{2-11} 
                                & \multirow{10}{*}{64} & 1                   & 0          & 5.1   & 0.05 & 0.15 & 0.41 & 0.23 & 0.01 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 13.91 & 0.01 & 0.01 & 8.84 & 4.55 & 0.01 & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 5.12  & 0.04 & 0.03 & 1.97 & 1.3  & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.87  & 0.02 & 0.02 & 0.78 & 0.7  & 0.01 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 16.69 & 0.21 & 0.35 & 9.64 & 4.48 & 0.05 & 0.03 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 2.75  & 0.03 & 0.03 & 0.79 & 0.68 & 0.01 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.82  & 0.02 & 0.02 & 0.66 & 0.57 & 0.01 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 19.16 & 0.23 & 0.35 & 10.9 & 5.14 & 0.06 & 0.03 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.4   & 0    & 0    & 0.46 & 0.46 & 0.01 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.5   & 0.01 & 0.01 & 0.52 & 0.48 & 0.01 & 0.01 \\ \hline
\multirow{10}{*}{Translational} & \multirow{10}{*}{64} & 1                   & 0          & 4.76  & 0.71 & 0.46 & 0.36 & 0.37 & 1.09 & 0.59 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.01  & 1.86 & 1.74 & 0.41 & 0.32 & 1.05 & 1.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0     & 0.23 & 0.37 & 0.22 & 0.24 & 0.22 & 0.2  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0     & 0.03 & 0.02 & 0    & 0    & 0.14 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.01  & 1.3  & 1.58 & 0.29 & 0.27 & 1.18 & 0.79 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0     & 0.23 & 0.47 & 0.19 & 0.2  & 0.4  & 0.39 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0     & 0.05 & 0.06 & 0.01 & 0.03 & 0.17 & 0.06 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 0.01  & 0.75 & 1.28 & 0.05 & 0.15 & 1.32 & 0.52 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0     & 0.22 & 0.6  & 0.18 & 0.18 & 0.85 & 0.43 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0     & 0.06 & 0.15 & 0.03 & 0.09 & 0.26 & 0.18 \\ \hline
\end{tabular}
\label{tab:fb15k-237_1}
\caption{Hits @ 1 \% results for complex query structures on FB15k-237. }
\end{table}



==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/fb15k-237_10.tex <==
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 16                   & 1                   & 0          & 18.48 & 0.17 & 0.27 & 1.32  & 0.94  & 0.09  & 0.08 \\ \cline{2-11} 
                                & 32                   & 1                   & 0          & 19.91 & 0.13 & 0.19 & 1.72  & 1.15  & 0.06  & 0.07 \\ \cline{2-11} 
                                & \multirow{10}{*}{64} & 1                   & 0          & 21.25 & 0.32 & 0.67 & 2.48  & 1.44  & 0.09  & 0.11 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 33.19 & 0.07 & 0.08 & 29.88 & 20    & 0.07  & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 14.7  & 0.15 & 0.14 & 9.96  & 8.12  & 0.09  & 0.1  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 5.88  & 0.11 & 0.11 & 3.14  & 3.28  & 0.07  & 0.08 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 35.11 & 0.67 & 1.03 & 31.9  & 20.77 & 0.21  & 0.21 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 9.45  & 0.12 & 0.12 & 4.74  & 4.34  & 0.07  & 0.09 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 5.24  & 0.1  & 0.09 & 3.19  & 3.31  & 0.07  & 0.07 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 36.21 & 0.8  & 1.25 & 33.17 & 21.06 & 0.25  & 0.26 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.71  & 0.04 & 0.04 & 1.76  & 2     & 0.07  & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.74  & 0.06 & 0.05 & 1.84  & 1.79  & 0.08  & 0.07 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{64} & 1                   & 0          & 21.46 & 3.65 & 3.07 & 3.23  & 3.01  & 6.67  & 4.75 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 31.53 & 7.79 & 7.5  & 3.36  & 2.63  & 9.77  & 7.47 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 9.52  & 1.77 & 1.8  & 1.57  & 1.74  & 1.66  & 1.71 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.33  & 0.12 & 0.1  & 0.1   & 0.09  & 0.22  & 0.14 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 31.2  & 8.45 & 8.03 & 3.38  & 2.69  & 10.67 & 7.82 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 11.71 & 2.75 & 2.75 & 2.2   & 2.15  & 3.82  & 3.81 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 3.12  & 0.4  & 0.38 & 0.79  & 1.05  & 0.6   & 0.83 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 30.69 & 9.67 & 8.81 & 3.22  & 2.67  & 12.33 & 8.25 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 11.99 & 4.45 & 4.21 & 2.67  & 2.69  & 7.28  & 5.71 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 4     & 0.94 & 0.85 & 1.73  & 2.27  & 1.69  & 2.22 \\ \hline
\end{tabular}
\label{tab:fb15k-237_10}
\caption{Hits @ 10 \% results for complex query structures on FB15k-237. }
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/fb15k-237_mrr.tex <==
\begin{table}[htbp]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{11}{*}{Shv}  & 16                   & 1                   & 0          & 8.62  & 0.08 & 0.09 & 0.57  & 0.38  & 0.05 & 0.05 \\ \cline{2-11} 
                                & 32                   & 1                   & 0          & 9.44  & 0.08 & 0.08 & 0.92  & 0.58  & 0.06 & 0.06 \\ \cline{2-11} 
                                & \multirow{9}{*}{64}  & 1                   & 0          & 10.16 & 0.08 & 0.08 & 1.16  & 0.69  & 0.06 & 0.06 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 20.28 & 0.07 & 0.08 & 15.95 & 10.04 & 0.07 & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 16.7  & 0.07 & 0.07 & 10.18 & 6.86  & 0.07 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 6.13  & 0.07 & 0.07 & 3.05  & 2.95  & 0.07 & 0.07 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 22.89 & 0.07 & 0.08 & 17.05 & 9.94  & 0.07 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 9.18  & 0.07 & 0.07 & 3.75  & 2.93  & 0.07 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 5.76  & 0.07 & 0.07 & 2.64  & 2.53  & 0.07 & 0.07 \\ \cline{3-11} 
                                &                      & \multirow{2}{*}{64} & 0          & 24.7  & 0.07 & 0.08 & 18.74 & 11.06 & 0.07 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.49  & 0.07 & 0.08 & 0.43  & 0.46  & 0.07 & 0.07 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{64} & 1                   & 0          & 10.16 & 1.88 & 1.48 & 1.52  & 1.44  & 3.18 & 2.38 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 10.9  & 4.02 & 3.77 & 1.34  & 1.06  & 4.15 & 3.51 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.21  & 0.84 & 0.94 & 0.62  & 0.68  & 0.78 & 0.66 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.59  & 0.1  & 0.08 & 0.07  & 0.08  & 0.21 & 0.1  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 10.93 & 3.91 & 3.86 & 1.3   & 1.09  & 4.52 & 3.36 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.93  & 1.21 & 1.35 & 0.85  & 0.86  & 1.65 & 1.67 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.21  & 0.21 & 0.21 & 0.26  & 0.33  & 0.38 & 0.36 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 10.9  & 3.98 & 3.93 & 1.08  & 1     & 5.17 & 3.28 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 4.16  & 1.82 & 1.95 & 1.03  & 1     & 3.01 & 2.38 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.46  & 0.42 & 0.44 & 0.56  & 0.84  & 0.81 & 0.96 \\ \hline
\end{tabular}
\label{tab:fb15k-237_mrr}
\caption{MRR \% results for complex query structures on FB15k-237. }
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/fb15k-237_mrr_std.tex <==
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 16                   & 1                   & 0          & 0.16 & 0.06 & 0.11 & 0.23 & 0.19 & 0.01 & 0.01 \\ \cline{2-11} 
                                & 32                   & 1                   & 0          & 0.11 & 0.02 & 0.03 & 0.08 & 0.07 & 0.01 & 0.01 \\ \cline{2-11} 
                                & \multirow{10}{*}{64} & 1                   & 0          & 0.04 & 0.02 & 0.09 & 0.09 & 0.09 & 0.01 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.24 & 0    & 0    & 0.12 & 0.21 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 7.28 & 0.04 & 0.03 & 4.78 & 2.78 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 2.5  & 0.02 & 0.02 & 1.15 & 1.05 & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.1  & 0.32 & 0.52 & 0.21 & 0.41 & 0.07 & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.64 & 0.03 & 0.02 & 1.22 & 0.7  & 0.01 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 2.39 & 0.01 & 0.01 & 0.91 & 0.82 & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 0.13 & 0.28 & 0.44 & 0.41 & 0.45 & 0.07 & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.07 & 0.01 & 0.01 & 0.32 & 0.36 & 0    & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02 & 0.01 & 0.01 & 0.05 & 0.06 & 0    & 0    \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{64} & 1                   & 0          & 0.01 & 0.1  & 0.04 & 0.07 & 0.05 & 0.07 & 0.05 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.05 & 0.02 & 0.05 & 0.04 & 0.01 & 0.17 & 0.14 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.01 & 0.02 & 0.01 & 0.07 & 0.07 & 0.05 & 0.18 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02 & 0    & 0    & 0.01 & 0    & 0    & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.1  & 0.01 & 0.05 & 0.06 & 0.1  & 0.09 & 0.13 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.03 & 0.05 & 0.03 & 0.01 & 0.02 & 0.06 & 0.05 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.06 & 0    & 0    & 0.02 & 0.03 & 0.02 & 0.02 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 0.07 & 0.11 & 0.15 & 0    & 0.02 & 0.12 & 0.11 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.04 & 0.03 & 0.02 & 0.02 & 0.03 & 0.09 & 0.05 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.04 & 0.01 & 0.01 & 0.01 & 0.06 & 0.02 & 0.05 \\ \hline
\end{tabular}
\label{tab:fb15k-237_mrr_std}
\caption{Standard deviation of MRR (\%) results for complex query structures on FB15k-237. }
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/hard/naive_vs_extension_hits_at_10.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
    dataset & model & 2p & 3p & 2i & 3i & pi & ip \\ \hline
    NELL-995 & ExtensionTransE & 0.101 & 0.087 & 0.298 & 0.393 & 0.198 & 0.124 \\ 
    ~ & NaiveTransE & 0.086 & 0.060 & 0.308 & 0.402 & 0.173 & 0.088 \\ \hline
    FB15k-237 & ExtensionTransE & 0.049 & 0.028 & 0.213 & 0.312 & 0.158 & 0.086 \\ 
    ~ & NaiveTransE & 0.049 & 0.024 & 0.213 & 0.307 & 0.142 & 0.045 \\ \hline
\end{tabular}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/hard/naive_vs_extension_mrr.tex <==
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
    dataset & model & 2p & 3p & 2i & 3i & pi & ip \\ \hline
    NELL-995 & ExtensionTransE & \textbf{0.060} & \textbf{0.054} & \textbf{0.165} & 0.234 & \textbf{0.126} & \textbf{0.079} \\ 
    ~ & NaiveTransE & 0.055 & 0.042 & 0.158 & \textbf{0.238} & 0.105 & 0.049 \\ \hline
    FB15k-237 & ExtensionTransE & 0.022 & \textbf{0.015} & \textbf{0.100} & \textbf{0.154} & \textbf{0.074} & \textbf{0.044} \\
    ~ & NaiveTransE & \textbf{0.025} & 0.013 & 0.093 & 0.153 & 0.064 & 0.024 \\ \hline
\end{tabular}}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/naive_vs_extension_FB15k-237.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
    \hline
        model & Metric & 1p & 2p & 3p & 2i & 3i & pi & ip \\ \hline
        ExtensionTransE & Hits@1 & 0.179 & 0.039 & 0.023 & 0.065 & 0.066 & 0.054 & 0.061 \\ 
        ~ & Hits@10 & 0.640 & 0.166 & 0.102 & 0.337 & 0.349 & 0.256 & 0.207 \\ 
        ~ & MRR & 0.326 & 0.083 & 0.053 & 0.152 & 0.156 & 0.122 & 0.112 \\ \hline
        NaiveTransE & Hits@1 & 0.188 & 0.039 & 0.025 & 0.060 & 0.071 & 0.045 & 0.022 \\ 
        ~ & Hits@10 & 0.657 & 0.161 & 0.096 & 0.356 & 0.365 & 0.229 & 0.099 \\ 
        ~ & MRR & 0.339 & 0.080 & 0.052 & 0.154 & 0.164 & 0.107 & 0.050 \\ \hline
    \end{tabular}
    \caption{Comparative performance of the extension and naive TransE approaches on FB15k-237.} 
    \label{tab:transe_traversal_fb15k-237}
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/naive_vs_extension_NELL.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
    \hline
        model & Metric & 1p & 2p & 3p & 2i & 3i & pi & ip  \\ \hline
        ExtensionTransE & Hits@1 & 0.367 & 0.176 & 0.081 & 0.184 & 0.114 & 0.256 & 0.231  \\
        ~ & Hits@10 & 0.700 & 0.349 & 0.220 & 0.464 & 0.385 & 0.499 & 0.438  \\
        ~ & MRR & 0.483 & 0.235 & 0.129 & 0.280 & 0.201 & 0.336 & 0.302  \\ \hline
        NaiveTransE & Hits@1 & 0.336 & 0.055 & 0.029 & 0.161 & 0.106 & 0.114 & 0.028  \\ 
        ~ & Hits@10 & 0.790 & 0.187 & 0.103 & 0.504 & 0.412 & 0.373 & 0.144  \\ 
        ~ & MRR & 0.500 & 0.101 & 0.053 & 0.274 & 0.207 & 0.200 & 0.069 \\ \hline
    \end{tabular}
    \caption{Comparative performance of the extension and naive TransE approaches on NELL-995.}
    \label{tab:transe_traversal_nell}
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/naive_vs_extension_easy_and_hard_hits_at_10.tex <==
\begin{table}[!ht]
    \centering
    \input{tables/easy/naive_vs_extension_hits_at_10} \\
    \vspace{1em}
    \input{tables/hard/naive_vs_extension_hits_at_10}
\caption{Comparative H@10 performance of the extension and naive TransE approaches for ``easy'' (top) and ``hard'' (bottom) complex query answers on NELL and FB15k-237 datasets.} 
\label{tab:transe_traversal_easy}
\end{table}


==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/naive_vs_extension_easy_and_hard_mrr.tex <==
\begin{table}[!ht]
    \centering
    \include{tables/easy/naive_vs_extension_mrr}
    \include{tables/hard/naive_vs_extension_mrr}
\caption{Comparative MRR performance of the extension and naive TransE approaches for ``easy'' (top) and ``hard'' (bottom) complex query answers on NELL-995 and FB15k-237 datasets.} 
\label{tab:transe_traversal_mrr}
\end{table}


==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/nell995_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                  & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 8                    & 1                   & 0          & 7.16  & 0    & 0.01 & 0.03 & 0.01 & 0    & 0    \\ \cline{2-11} 
                                & 16                   & 1                   & 0          & 8.78  & 0    & 0    & 0.09 & 0.06 & 0    & 0    \\ \cline{2-11} 
                                & \multirow{10}{*}{32} & 1                   & 0          & 9.89  & 0    & 0    & 0.19 & 0.15 & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 24.45 & 0    & 0    & 2.19 & 1.83 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.93  & 0.33 & 0.32 & 0.61 & 0.67 & 0.11 & 0.2  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 2.11  & 0.13 & 0.13 & 0.4  & 0.46 & 0.04 & 0.12 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 26.64 & 0    & 0    & 2.27 & 1.77 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.55  & 0.28 & 0.28 & 0.6  & 0.6  & 0.09 & 0.2  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.56  & 0.12 & 0.11 & 0.35 & 0.42 & 0.03 & 0.12 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 29.33 & 0    & 0    & 2.28 & 1.99 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.57  & 0    & 0    & 0.07 & 0.04 & 0    & 0.09 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.51  & 0    & 0    & 0.05 & 0.03 & 0    & 0.13 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{32} & 1                   & 0          & 12.46 & 0    & 0    & 3.14 & 2.44 & 0    & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 0.06  & 0.03 & 0    & 2.29 & 2.32 & 0.2  & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.02  & 0.02 & 0    & 0.3  & 0.33 & 0.2  & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02  & 0.02 & 0    & 0.02 & 0.03 & 0.21 & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.06  & 0.05 & 0.01 & 1.2  & 1.24 & 0.22 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.03  & 0.05 & 0.01 & 0.21 & 0.21 & 0.21 & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02  & 0.06 & 0    & 0.02 & 0.03 & 0.21 & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.07  & 0.08 & 0.02 & 0.68 & 1.15 & 0.22 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.08  & 0.07 & 0.02 & 0.18 & 0.15 & 0.21 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02  & 0.1  & 0.02 & 0.02 & 0.02 & 0.21 & 0.01 \\ \hline
\end{tabular}
\label{tab:nell995_1}
\caption{Hits @ 1 \% results for complex query structures on NELL995. }
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/nell995_10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                  & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 8                    & 1                   & 0          & 30.56 & 0.01 & 0.09 & 0.24  & 0.17  & 0.01 & 0    \\ \cline{2-11} 
                                & 16                   & 1                   & 0          & 34.25 & 0.01 & 0.01 & 0.62  & 0.5   & 0.01 & 0    \\ \cline{2-11} 
                                & \multirow{10}{*}{32} & 1                   & 0          & 36.91 & 0.01 & 0.02 & 1.05  & 0.85  & 0.02 & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 61.23 & 0.02 & 0.02 & 11.56 & 11.12 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 10.55 & 0.61 & 0.54 & 2.83  & 3.51  & 0.26 & 0.7  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 4.94  & 0.24 & 0.23 & 0.9   & 1.12  & 0.08 & 0.31 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 62.65 & 0.02 & 0.02 & 11.87 & 11.11 & 0.02 & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 8.82  & 0.5  & 0.45 & 2.2   & 2.74  & 0.2  & 0.67 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 3.59  & 0.2  & 0.19 & 0.72  & 0.88  & 0.07 & 0.31 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 64.55 & 0.02 & 0.02 & 11.98 & 11.31 & 0.02 & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 1.14  & 0.02 & 0.01 & 0.22  & 0.15  & 0.02 & 0.3  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.98  & 0.02 & 0.02 & 0.17  & 0.1   & 0.02 & 0.36 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{32} & 1                   & 0          & 34.13 & 0.01 & 0.01 & 15.92 & 14.05 & 0.03 & 0.4  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 37.47 & 0.06 & 0.01 & 21.21 & 22.94 & 0.24 & 0.09 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 5.75  & 0.04 & 0    & 1.84  & 2.4   & 0.22 & 0.02 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.25  & 0.05 & 0.01 & 0.07  & 0.07  & 0.22 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 35.75 & 0.07 & 0.02 & 20.82 & 22.76 & 0.24 & 0.09 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 10.6  & 0.06 & 0.02 & 2.59  & 2.47  & 0.22 & 0.04 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.3   & 0.08 & 0.02 & 0.07  & 0.06  & 0.22 & 0.03 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 37.72 & 0.1  & 0.03 & 21.94 & 23.2  & 0.24 & 0.12 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 25.27 & 0.1  & 0.04 & 5.84  & 2.16  & 0.23 & 0.17 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.5   & 0.11 & 0.03 & 0.1   & 0.1   & 0.22 & 0.06 \\ \hline
\end{tabular}
\label{tab:nell995_10}
\caption{Hits @ 10 \% results for complex query structures on NELL995. }
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/nell995_mrr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                  & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 8                    & 1                   & 0          & 14.9  & 0.01 & 0.06 & 0.15 & 0.11 & 0.01 & 0    \\ \cline{2-11} 
                                & 16                   & 1                   & 0          & 17.21 & 0.01 & 0.02 & 0.33 & 0.28 & 0.01 & 0    \\ \cline{2-11} 
                                & \multirow{10}{*}{32} & 1                   & 0          & 18.78 & 0.01 & 0.02 & 0.58 & 0.5  & 0.02 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 36.39 & 0.02 & 0.02 & 5.3  & 4.85 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 6.19  & 0.45 & 0.42 & 1.37 & 1.58 & 0.18 & 0.4  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 3.1   & 0.19 & 0.18 & 0.6  & 0.72 & 0.07 & 0.2  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 38.48 & 0.02 & 0.02 & 5.47 & 4.84 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 5.35  & 0.38 & 0.36 & 1.19 & 1.35 & 0.14 & 0.39 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 2.27  & 0.16 & 0.15 & 0.5  & 0.6  & 0.06 & 0.2  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 40.94 & 0.02 & 0.02 & 5.51 & 5.09 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.79  & 0.02 & 0.02 & 0.14 & 0.1  & 0.02 & 0.18 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.69  & 0.02 & 0.02 & 0.11 & 0.07 & 0.02 & 0.23 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{32} & 1                   & 0          & 19.65 & 0.01 & 0.01 & 7.51 & 6.44 & 0.03 & 0.16 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 12.18 & 0.04 & 0.01 & 8.53 & 8.94 & 0.22 & 0.05 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 2.18  & 0.03 & 0.01 & 0.98 & 1.2  & 0.21 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.12  & 0.04 & 0.01 & 0.05 & 0.06 & 0.23 & 0.02 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 11.84 & 0.06 & 0.01 & 7.26 & 7.81 & 0.23 & 0.05 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.84  & 0.06 & 0.01 & 1.18 & 1.18 & 0.22 & 0.03 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.14  & 0.07 & 0.02 & 0.05 & 0.06 & 0.22 & 0.02 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 12.6  & 0.09 & 0.03 & 6.91 & 7.63 & 0.23 & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 10.24 & 0.09 & 0.03 & 2.06 & 1    & 0.22 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.21  & 0.11 & 0.03 & 0.06 & 0.06 & 0.22 & 0.04 \\ \hline
\end{tabular}
\label{tab:nell995_mrr}
\caption{MRR \% results for complex query structures on NELL995. }
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/nell995_mrr_std.tex <==
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 8                    & 1                   & 0          & 0.14  & 0    & 0.02 & 0.05 & 0.01 & 0    & 0    \\ \cline{2-11} 
                                & 16                   & 1                   & 0          & 0.22  & 0    & 0    & 0.03 & 0.01 & 0    & 0    \\ \cline{2-11} 
                                & \multirow{10}{*}{32} & 1                   & 0          & 0.16  & 0    & 0    & 0.07 & 0.1  & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 0.29  & 0    & 0    & 0.05 & 0.28 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.16  & 0.21 & 0.2  & 0.04 & 0.05 & 0.08 & 0.19 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.25  & 0.08 & 0.08 & 0.02 & 0.03 & 0.02 & 0.1  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.23  & 0    & 0    & 0.09 & 0.12 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.15  & 0.18 & 0.17 & 0.03 & 0.02 & 0.06 & 0.18 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.17  & 0.07 & 0.07 & 0.03 & 0.06 & 0.02 & 0.09 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.25  & 0    & 0    & 0.08 & 0.29 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.01  & 0.01 & 0    & 0.01 & 0.01 & 0    & 0.08 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.03  & 0    & 0    & 0.01 & 0.01 & 0    & 0.11 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{32} & 1                   & 0          & 16.96 & 0.01 & 0.01 & 6.46 & 5.54 & 0.01 & 0.12 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 0.14  & 0    & 0    & 0.12 & 0.31 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.08  & 0    & 0    & 0.11 & 0.17 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.06  & 0    & 0    & 0.01 & 0.02 & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.06  & 0    & 0    & 0.08 & 0.15 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.09  & 0    & 0    & 0.05 & 0.03 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02  & 0    & 0    & 0    & 0    & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.06  & 0    & 0    & 0.09 & 0.09 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.03  & 0    & 0.01 & 0.03 & 0    & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.01  & 0    & 0    & 0    & 0    & 0    & 0    \\ \hline
\end{tabular}
\label{tab:nell995_mrr_std}
\caption{Standard deviation of MRR (\%) results for complex query structures on NELL995.}
\end{table}

==> A Sheaf-Theoretic Framework for Knowledge Graph Embedding/tables/transe_traversal.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lrrrrrrr}
\toprule
{} &     1p &    2p &    3p &    2i &    3i &    ip &    pi \\
\midrule
H@1   &   4.76 &  0.64 &  0.28 &  0.46 &  0.32 &  0.45 &  0.23 \\
% H@3   &  11.57 &  1.37 &  0.61 &  1.43 &  1.04 &  0.96 &  0.70 \\
% H@5   &  15.57 &  1.91 &  0.87 &  2.33 &  1.82 &  1.47 &  1.19 \\
H@10  &  21.46 &  2.85 &  1.38 &  4.32 &  3.93 &  2.75 &  2.65 \\
MRR &  10.16 &  1.48 &  0.75 &  1.90 &  1.80 &  1.29 &  1.29 \\
\bottomrule
\end{tabular}
\label{tab:transe_traversal}
\caption{Results (\%) for naive complex query answering approach for ShvT model with 64 embedding dimensions and 1 section on FB15k-237.}
\end{table}

==> tables/fb15k-237_1.tex <==
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Multisection}  & 16                   & 1                   & 0          & 4.03  & 0.03 & 0.04 & 0.2  & 0.15 & 0.01 & 0.01 \\ \cline{2-11} 
                                & 32                   & 1                   & 0          & 4.65  & 0.01 & 0.02 & 0.28 & 0.18 & 0.01 & 0.01 \\ \cline{2-11} 
                                & \multirow{10}{*}{64} & 1                   & 0          & 5.1   & 0.05 & 0.15 & 0.41 & 0.23 & 0.01 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 13.91 & 0.01 & 0.01 & 8.84 & 4.55 & 0.01 & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 5.12  & 0.04 & 0.03 & 1.97 & 1.3  & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.87  & 0.02 & 0.02 & 0.78 & 0.7  & 0.01 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 16.69 & 0.21 & 0.35 & 9.64 & 4.48 & 0.05 & 0.03 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 2.75  & 0.03 & 0.03 & 0.79 & 0.68 & 0.01 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.82  & 0.02 & 0.02 & 0.66 & 0.57 & 0.01 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 19.16 & 0.23 & 0.35 & 10.9 & 5.14 & 0.06 & 0.03 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.4   & 0    & 0    & 0.46 & 0.46 & 0.01 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.5   & 0.01 & 0.01 & 0.52 & 0.48 & 0.01 & 0.01 \\ \hline
\multirow{10}{*}{Translational} & \multirow{10}{*}{64} & 1                   & 0          & 4.76  & 0.71 & 0.46 & 0.36 & 0.37 & 1.09 & 0.59 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.01  & 1.86 & 1.74 & 0.41 & 0.32 & 1.05 & 1.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0     & 0.23 & 0.37 & 0.22 & 0.24 & 0.22 & 0.2  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0     & 0.03 & 0.02 & 0    & 0    & 0.14 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.01  & 1.3  & 1.58 & 0.29 & 0.27 & 1.18 & 0.79 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0     & 0.23 & 0.47 & 0.19 & 0.2  & 0.4  & 0.39 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0     & 0.05 & 0.06 & 0.01 & 0.03 & 0.17 & 0.06 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 0.01  & 0.75 & 1.28 & 0.05 & 0.15 & 1.32 & 0.52 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0     & 0.22 & 0.6  & 0.18 & 0.18 & 0.85 & 0.43 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0     & 0.06 & 0.15 & 0.03 & 0.09 & 0.26 & 0.18 \\ \hline
\end{tabular}
\label{tab:fb15k-237_1}
\caption{Hits @ 1 \% results for complex query structures on FB15k-237. }
\end{table}



==> tables/fb15k-237_10.tex <==
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 16                   & 1                   & 0          & 18.48 & 0.17 & 0.27 & 1.32  & 0.94  & 0.09  & 0.08 \\ \cline{2-11} 
                                & 32                   & 1                   & 0          & 19.91 & 0.13 & 0.19 & 1.72  & 1.15  & 0.06  & 0.07 \\ \cline{2-11} 
                                & \multirow{10}{*}{64} & 1                   & 0          & 21.25 & 0.32 & 0.67 & 2.48  & 1.44  & 0.09  & 0.11 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 33.19 & 0.07 & 0.08 & 29.88 & 20    & 0.07  & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 14.7  & 0.15 & 0.14 & 9.96  & 8.12  & 0.09  & 0.1  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 5.88  & 0.11 & 0.11 & 3.14  & 3.28  & 0.07  & 0.08 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 35.11 & 0.67 & 1.03 & 31.9  & 20.77 & 0.21  & 0.21 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 9.45  & 0.12 & 0.12 & 4.74  & 4.34  & 0.07  & 0.09 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 5.24  & 0.1  & 0.09 & 3.19  & 3.31  & 0.07  & 0.07 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 36.21 & 0.8  & 1.25 & 33.17 & 21.06 & 0.25  & 0.26 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.71  & 0.04 & 0.04 & 1.76  & 2     & 0.07  & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.74  & 0.06 & 0.05 & 1.84  & 1.79  & 0.08  & 0.07 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{64} & 1                   & 0          & 21.46 & 3.65 & 3.07 & 3.23  & 3.01  & 6.67  & 4.75 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 31.53 & 7.79 & 7.5  & 3.36  & 2.63  & 9.77  & 7.47 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 9.52  & 1.77 & 1.8  & 1.57  & 1.74  & 1.66  & 1.71 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.33  & 0.12 & 0.1  & 0.1   & 0.09  & 0.22  & 0.14 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 31.2  & 8.45 & 8.03 & 3.38  & 2.69  & 10.67 & 7.82 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 11.71 & 2.75 & 2.75 & 2.2   & 2.15  & 3.82  & 3.81 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 3.12  & 0.4  & 0.38 & 0.79  & 1.05  & 0.6   & 0.83 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 30.69 & 9.67 & 8.81 & 3.22  & 2.67  & 12.33 & 8.25 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 11.99 & 4.45 & 4.21 & 2.67  & 2.69  & 7.28  & 5.71 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 4     & 0.94 & 0.85 & 1.73  & 2.27  & 1.69  & 2.22 \\ \hline
\end{tabular}
\label{tab:fb15k-237_10}
\caption{Hits @ 10 \% results for complex query structures on FB15k-237. }
\end{table}

==> tables/fb15k-237_mrr.tex <==
\begin{table}[htbp]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{11}{*}{Shv}  & 16                   & 1                   & 0          & 8.62  & 0.08 & 0.09 & 0.57  & 0.38  & 0.05 & 0.05 \\ \cline{2-11} 
                                & 32                   & 1                   & 0          & 9.44  & 0.08 & 0.08 & 0.92  & 0.58  & 0.06 & 0.06 \\ \cline{2-11} 
                                & \multirow{9}{*}{64}  & 1                   & 0          & 10.16 & 0.08 & 0.08 & 1.16  & 0.69  & 0.06 & 0.06 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 20.28 & 0.07 & 0.08 & 15.95 & 10.04 & 0.07 & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 16.7  & 0.07 & 0.07 & 10.18 & 6.86  & 0.07 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 6.13  & 0.07 & 0.07 & 3.05  & 2.95  & 0.07 & 0.07 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 22.89 & 0.07 & 0.08 & 17.05 & 9.94  & 0.07 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 9.18  & 0.07 & 0.07 & 3.75  & 2.93  & 0.07 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 5.76  & 0.07 & 0.07 & 2.64  & 2.53  & 0.07 & 0.07 \\ \cline{3-11} 
                                &                      & \multirow{2}{*}{64} & 0          & 24.7  & 0.07 & 0.08 & 18.74 & 11.06 & 0.07 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.49  & 0.07 & 0.08 & 0.43  & 0.46  & 0.07 & 0.07 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{64} & 1                   & 0          & 10.16 & 1.88 & 1.48 & 1.52  & 1.44  & 3.18 & 2.38 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 10.9  & 4.02 & 3.77 & 1.34  & 1.06  & 4.15 & 3.51 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.21  & 0.84 & 0.94 & 0.62  & 0.68  & 0.78 & 0.66 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.59  & 0.1  & 0.08 & 0.07  & 0.08  & 0.21 & 0.1  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 10.93 & 3.91 & 3.86 & 1.3   & 1.09  & 4.52 & 3.36 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.93  & 1.21 & 1.35 & 0.85  & 0.86  & 1.65 & 1.67 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.21  & 0.21 & 0.21 & 0.26  & 0.33  & 0.38 & 0.36 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 10.9  & 3.98 & 3.93 & 1.08  & 1     & 5.17 & 3.28 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 4.16  & 1.82 & 1.95 & 1.03  & 1     & 3.01 & 2.38 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.46  & 0.42 & 0.44 & 0.56  & 0.84  & 0.81 & 0.96 \\ \hline
\end{tabular}
\label{tab:fb15k-237_mrr}
\caption{MRR \% results for complex query structures on FB15k-237. }
\end{table}

==> tables/fb15k-237_mrr_std.tex <==
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 16                   & 1                   & 0          & 0.16 & 0.06 & 0.11 & 0.23 & 0.19 & 0.01 & 0.01 \\ \cline{2-11} 
                                & 32                   & 1                   & 0          & 0.11 & 0.02 & 0.03 & 0.08 & 0.07 & 0.01 & 0.01 \\ \cline{2-11} 
                                & \multirow{10}{*}{64} & 1                   & 0          & 0.04 & 0.02 & 0.09 & 0.09 & 0.09 & 0.01 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.24 & 0    & 0    & 0.12 & 0.21 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 7.28 & 0.04 & 0.03 & 4.78 & 2.78 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 2.5  & 0.02 & 0.02 & 1.15 & 1.05 & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.1  & 0.32 & 0.52 & 0.21 & 0.41 & 0.07 & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.64 & 0.03 & 0.02 & 1.22 & 0.7  & 0.01 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 2.39 & 0.01 & 0.01 & 0.91 & 0.82 & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 0.13 & 0.28 & 0.44 & 0.41 & 0.45 & 0.07 & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.07 & 0.01 & 0.01 & 0.32 & 0.36 & 0    & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02 & 0.01 & 0.01 & 0.05 & 0.06 & 0    & 0    \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{64} & 1                   & 0          & 0.01 & 0.1  & 0.04 & 0.07 & 0.05 & 0.07 & 0.05 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.05 & 0.02 & 0.05 & 0.04 & 0.01 & 0.17 & 0.14 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.01 & 0.02 & 0.01 & 0.07 & 0.07 & 0.05 & 0.18 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02 & 0    & 0    & 0.01 & 0    & 0    & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.1  & 0.01 & 0.05 & 0.06 & 0.1  & 0.09 & 0.13 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.03 & 0.05 & 0.03 & 0.01 & 0.02 & 0.06 & 0.05 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.06 & 0    & 0    & 0.02 & 0.03 & 0.02 & 0.02 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{64} & 0          & 0.07 & 0.11 & 0.15 & 0    & 0.02 & 0.12 & 0.11 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.04 & 0.03 & 0.02 & 0.02 & 0.03 & 0.09 & 0.05 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.04 & 0.01 & 0.01 & 0.01 & 0.06 & 0.02 & 0.05 \\ \hline
\end{tabular}
\label{tab:fb15k-237_mrr_std}
\caption{Standard deviation of MRR (\%) results for complex query structures on FB15k-237. }
\end{table}

==> tables/naive_vs_extension_FB15k-237.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
    \hline
        model & Metric & 1p & 2p & 3p & 2i & 3i & pi & ip \\ \hline
        ExtensionTransE & Hits@1 & 0.179 & 0.039 & 0.023 & 0.065 & 0.066 & 0.054 & 0.061 \\ 
        ~ & Hits@10 & 0.640 & 0.166 & 0.102 & 0.337 & 0.349 & 0.256 & 0.207 \\ 
        ~ & MRR & 0.326 & 0.083 & 0.053 & 0.152 & 0.156 & 0.122 & 0.112 \\ \hline
        NaiveTransE & Hits@1 & 0.188 & 0.039 & 0.025 & 0.060 & 0.071 & 0.045 & 0.022 \\ 
        ~ & Hits@10 & 0.657 & 0.161 & 0.096 & 0.356 & 0.365 & 0.229 & 0.099 \\ 
        ~ & MRR & 0.339 & 0.080 & 0.052 & 0.154 & 0.164 & 0.107 & 0.050 \\ \hline
    \end{tabular}
    \caption{Comparative performance of the extension and naive TransE approaches on FB15k-237.} 
    \label{tab:transe_traversal_fb15k-237}
\end{table}

==> tables/naive_vs_extension_NELL.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
    \hline
        model & Metric & 1p & 2p & 3p & 2i & 3i & pi & ip  \\ \hline
        ExtensionTransE & Hits@1 & 0.367 & 0.176 & 0.081 & 0.184 & 0.114 & 0.256 & 0.231  \\
        ~ & Hits@10 & 0.700 & 0.349 & 0.220 & 0.464 & 0.385 & 0.499 & 0.438  \\
        ~ & MRR & 0.483 & 0.235 & 0.129 & 0.280 & 0.201 & 0.336 & 0.302  \\ \hline
        NaiveTransE & Hits@1 & 0.336 & 0.055 & 0.029 & 0.161 & 0.106 & 0.114 & 0.028  \\ 
        ~ & Hits@10 & 0.790 & 0.187 & 0.103 & 0.504 & 0.412 & 0.373 & 0.144  \\ 
        ~ & MRR & 0.500 & 0.101 & 0.053 & 0.274 & 0.207 & 0.200 & 0.069 \\ \hline
    \end{tabular}
    \caption{Comparative performance of the extension and naive TransE approaches on NELL-995.}
    \label{tab:transe_traversal_nell}
\end{table}

==> tables/nell995_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                  & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 8                    & 1                   & 0          & 7.16  & 0    & 0.01 & 0.03 & 0.01 & 0    & 0    \\ \cline{2-11} 
                                & 16                   & 1                   & 0          & 8.78  & 0    & 0    & 0.09 & 0.06 & 0    & 0    \\ \cline{2-11} 
                                & \multirow{10}{*}{32} & 1                   & 0          & 9.89  & 0    & 0    & 0.19 & 0.15 & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 24.45 & 0    & 0    & 2.19 & 1.83 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.93  & 0.33 & 0.32 & 0.61 & 0.67 & 0.11 & 0.2  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 2.11  & 0.13 & 0.13 & 0.4  & 0.46 & 0.04 & 0.12 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 26.64 & 0    & 0    & 2.27 & 1.77 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.55  & 0.28 & 0.28 & 0.6  & 0.6  & 0.09 & 0.2  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 1.56  & 0.12 & 0.11 & 0.35 & 0.42 & 0.03 & 0.12 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 29.33 & 0    & 0    & 2.28 & 1.99 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.57  & 0    & 0    & 0.07 & 0.04 & 0    & 0.09 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.51  & 0    & 0    & 0.05 & 0.03 & 0    & 0.13 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{32} & 1                   & 0          & 12.46 & 0    & 0    & 3.14 & 2.44 & 0    & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 0.06  & 0.03 & 0    & 2.29 & 2.32 & 0.2  & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.02  & 0.02 & 0    & 0.3  & 0.33 & 0.2  & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02  & 0.02 & 0    & 0.02 & 0.03 & 0.21 & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.06  & 0.05 & 0.01 & 1.2  & 1.24 & 0.22 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.03  & 0.05 & 0.01 & 0.21 & 0.21 & 0.21 & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02  & 0.06 & 0    & 0.02 & 0.03 & 0.21 & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.07  & 0.08 & 0.02 & 0.68 & 1.15 & 0.22 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.08  & 0.07 & 0.02 & 0.18 & 0.15 & 0.21 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02  & 0.1  & 0.02 & 0.02 & 0.02 & 0.21 & 0.01 \\ \hline
\end{tabular}
\label{tab:nell995_1}
\caption{Hits @ 1 \% results for complex query structures on NELL995. }
\end{table}

==> tables/nell995_10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                  & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 8                    & 1                   & 0          & 30.56 & 0.01 & 0.09 & 0.24  & 0.17  & 0.01 & 0    \\ \cline{2-11} 
                                & 16                   & 1                   & 0          & 34.25 & 0.01 & 0.01 & 0.62  & 0.5   & 0.01 & 0    \\ \cline{2-11} 
                                & \multirow{10}{*}{32} & 1                   & 0          & 36.91 & 0.01 & 0.02 & 1.05  & 0.85  & 0.02 & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 61.23 & 0.02 & 0.02 & 11.56 & 11.12 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 10.55 & 0.61 & 0.54 & 2.83  & 3.51  & 0.26 & 0.7  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 4.94  & 0.24 & 0.23 & 0.9   & 1.12  & 0.08 & 0.31 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 62.65 & 0.02 & 0.02 & 11.87 & 11.11 & 0.02 & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 8.82  & 0.5  & 0.45 & 2.2   & 2.74  & 0.2  & 0.67 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 3.59  & 0.2  & 0.19 & 0.72  & 0.88  & 0.07 & 0.31 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 64.55 & 0.02 & 0.02 & 11.98 & 11.31 & 0.02 & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 1.14  & 0.02 & 0.01 & 0.22  & 0.15  & 0.02 & 0.3  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.98  & 0.02 & 0.02 & 0.17  & 0.1   & 0.02 & 0.36 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{32} & 1                   & 0          & 34.13 & 0.01 & 0.01 & 15.92 & 14.05 & 0.03 & 0.4  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 37.47 & 0.06 & 0.01 & 21.21 & 22.94 & 0.24 & 0.09 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 5.75  & 0.04 & 0    & 1.84  & 2.4   & 0.22 & 0.02 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.25  & 0.05 & 0.01 & 0.07  & 0.07  & 0.22 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 35.75 & 0.07 & 0.02 & 20.82 & 22.76 & 0.24 & 0.09 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 10.6  & 0.06 & 0.02 & 2.59  & 2.47  & 0.22 & 0.04 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.3   & 0.08 & 0.02 & 0.07  & 0.06  & 0.22 & 0.03 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 37.72 & 0.1  & 0.03 & 21.94 & 23.2  & 0.24 & 0.12 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 25.27 & 0.1  & 0.04 & 5.84  & 2.16  & 0.23 & 0.17 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.5   & 0.11 & 0.03 & 0.1   & 0.1   & 0.22 & 0.06 \\ \hline
\end{tabular}
\label{tab:nell995_10}
\caption{Hits @ 10 \% results for complex query structures on NELL995. }
\end{table}

==> tables/nell995_mrr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                  & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 8                    & 1                   & 0          & 14.9  & 0.01 & 0.06 & 0.15 & 0.11 & 0.01 & 0    \\ \cline{2-11} 
                                & 16                   & 1                   & 0          & 17.21 & 0.01 & 0.02 & 0.33 & 0.28 & 0.01 & 0    \\ \cline{2-11} 
                                & \multirow{10}{*}{32} & 1                   & 0          & 18.78 & 0.01 & 0.02 & 0.58 & 0.5  & 0.02 & 0.01 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 36.39 & 0.02 & 0.02 & 5.3  & 4.85 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 6.19  & 0.45 & 0.42 & 1.37 & 1.58 & 0.18 & 0.4  \\ \cline{4-11} 
                                &                      &                     & 0.1        & 3.1   & 0.19 & 0.18 & 0.6  & 0.72 & 0.07 & 0.2  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 38.48 & 0.02 & 0.02 & 5.47 & 4.84 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 5.35  & 0.38 & 0.36 & 1.19 & 1.35 & 0.14 & 0.39 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 2.27  & 0.16 & 0.15 & 0.5  & 0.6  & 0.06 & 0.2  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 40.94 & 0.02 & 0.02 & 5.51 & 5.09 & 0.02 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.79  & 0.02 & 0.02 & 0.14 & 0.1  & 0.02 & 0.18 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.69  & 0.02 & 0.02 & 0.11 & 0.07 & 0.02 & 0.23 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{32} & 1                   & 0          & 19.65 & 0.01 & 0.01 & 7.51 & 6.44 & 0.03 & 0.16 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 12.18 & 0.04 & 0.01 & 8.53 & 8.94 & 0.22 & 0.05 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 2.18  & 0.03 & 0.01 & 0.98 & 1.2  & 0.21 & 0.01 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.12  & 0.04 & 0.01 & 0.05 & 0.06 & 0.23 & 0.02 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 11.84 & 0.06 & 0.01 & 7.26 & 7.81 & 0.23 & 0.05 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 3.84  & 0.06 & 0.01 & 1.18 & 1.18 & 0.22 & 0.03 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.14  & 0.07 & 0.02 & 0.05 & 0.06 & 0.22 & 0.02 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 12.6  & 0.09 & 0.03 & 6.91 & 7.63 & 0.23 & 0.06 \\ \cline{4-11} 
                                &                      &                     & 0.01       & 10.24 & 0.09 & 0.03 & 2.06 & 1    & 0.22 & 0.07 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.21  & 0.11 & 0.03 & 0.06 & 0.06 & 0.22 & 0.04 \\ \hline
\end{tabular}
\label{tab:nell995_mrr}
\caption{MRR \% results for complex query structures on NELL995. }
\end{table}

==> tables/nell995_mrr_std.tex <==
\begin{table}[hbt!]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{model}                           & \boldmath$\dim \Fc(r)$       & \textbf{Sections}        & \boldmath$\alpha$ & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{ip} & \textbf{pi} \\ \hline
\multirow{12}{*}{Shv}  & 8                    & 1                   & 0          & 0.14  & 0    & 0.02 & 0.05 & 0.01 & 0    & 0    \\ \cline{2-11} 
                                & 16                   & 1                   & 0          & 0.22  & 0    & 0    & 0.03 & 0.01 & 0    & 0    \\ \cline{2-11} 
                                & \multirow{10}{*}{32} & 1                   & 0          & 0.16  & 0    & 0    & 0.07 & 0.1  & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 0.29  & 0    & 0    & 0.05 & 0.28 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.16  & 0.21 & 0.2  & 0.04 & 0.05 & 0.08 & 0.19 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.25  & 0.08 & 0.08 & 0.02 & 0.03 & 0.02 & 0.1  \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.23  & 0    & 0    & 0.09 & 0.12 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.15  & 0.18 & 0.17 & 0.03 & 0.02 & 0.06 & 0.18 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.17  & 0.07 & 0.07 & 0.03 & 0.06 & 0.02 & 0.09 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.25  & 0    & 0    & 0.08 & 0.29 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.01  & 0.01 & 0    & 0.01 & 0.01 & 0    & 0.08 \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.03  & 0    & 0    & 0.01 & 0.01 & 0    & 0.11 \\ \hline
\multirow{10}{*}{ShvT} & \multirow{10}{*}{32} & 1                   & 0          & 16.96 & 0.01 & 0.01 & 6.46 & 5.54 & 0.01 & 0.12 \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{8}  & 0          & 0.14  & 0    & 0    & 0.12 & 0.31 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.08  & 0    & 0    & 0.11 & 0.17 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.06  & 0    & 0    & 0.01 & 0.02 & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{16} & 0          & 0.06  & 0    & 0    & 0.08 & 0.15 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.09  & 0    & 0    & 0.05 & 0.03 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.02  & 0    & 0    & 0    & 0    & 0    & 0    \\ \cline{3-11} 
                                &                      & \multirow{3}{*}{32} & 0          & 0.06  & 0    & 0    & 0.09 & 0.09 & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.01       & 0.03  & 0    & 0.01 & 0.03 & 0    & 0    & 0    \\ \cline{4-11} 
                                &                      &                     & 0.1        & 0.01  & 0    & 0    & 0    & 0    & 0    & 0    \\ \hline
\end{tabular}
\label{tab:nell995_mrr_std}
\caption{Standard deviation of MRR (\%) results for complex query structures on NELL995.}
\end{table}

==> tables/transe_traversal.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lrrrrrrr}
\toprule
{} &     1p &    2p &    3p &    2i &    3i &    ip &    pi \\
\midrule
H@1   &   4.76 &  0.64 &  0.28 &  0.46 &  0.32 &  0.45 &  0.23 \\
% H@3   &  11.57 &  1.37 &  0.61 &  1.43 &  1.04 &  0.96 &  0.70 \\
% H@5   &  15.57 &  1.91 &  0.87 &  2.33 &  1.82 &  1.47 &  1.19 \\
H@10  &  21.46 &  2.85 &  1.38 &  4.32 &  3.93 &  2.75 &  2.65 \\
MRR &  10.16 &  1.48 &  0.75 &  1.90 &  1.80 &  1.29 &  1.29 \\
\bottomrule
\end{tabular}
\label{tab:transe_traversal}
\caption{Results (\%) for naive complex query answering approach for ShvT model with 64 embedding dimensions and 1 section on FB15k-237.}
\end{table}
